Advances in losing

We survey recent developments in the theory of impartial combinatorial games in misere play, focusing on how the Sprague-Grundy theory of normal-play impartial games generalizes to misere play via the indistinguishability quotient construction.

==> macros.tex <==
\makeatletter

\newcounter{misere@cnt}
\newcounter{misere@pcnt}
\newcounter{misere@period}

\newcommand{\pretend}[3]{%
  \begin{tabular}{c}
  $\begin{array}{r|ccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
  \misere@prehdr{#2}
  \\ \hline
  \misere@pre{#2}{#3}
  \end{array}$ \vspace{0.25cm} \\
  #1
  \end{tabular}
}

\newcommand{\misere@prehdr}[1]{
  \setcounter{misere@period}{#1}
  \setcounter{misere@cnt}{0}
  \misere@buildprehdr
}

\def\misere@buildprehdr{
  & \arabic{misere@cnt}
  \stepcounter{misere@cnt}
  \ifnum\arabic{misere@cnt}<\arabic{misere@period}
    \let\next=\misere@buildprehdr
  \else
    \let\next=\relax
  \fi
  \next
}

\newcommand{\misere@pre}[2]{
  \setcounter{misere@period}{#1}
  \setcounter{misere@cnt}{0}
  \setcounter{misere@pcnt}{0}
  \misere@buildpre#2 @ 
}

\def\misere@buildpre#1 {%
  \ifx#1@
    \let\next=\relax%
  \else
    \misere@processpre{#1}%
    \let\next=\misere@buildpre%
  \fi%
  \next%
}

\def\misere@processpre#1{%
  \ifnum\arabic{misere@pcnt}=\arabic{misere@period}
    \setcounter{misere@pcnt}{0}
  \fi
  \ifnum\arabic{misere@pcnt}=0
    \ifnum\arabic{misere@cnt}>0
      \\
    \fi
    \arabic{misere@cnt}
  \fi
  & #1%
  \stepcounter{misere@cnt}%
  \stepcounter{misere@pcnt}%
}

\makeatother

